Identification of optimal prediction error Th\'evenin models of Li-ion cells using the MOLI approach

This report presents System Identification algorithms to estimate the dynamical model of Li-Oin cells. First the dependence of open circuit voltage (OCV) on the state of charge (SOC) is studied. thN battery equivalent model when a resistor is added to the circuit is stated. The discharge data is divided into segments where the internal resistance is assumed constant, and therefore SOC is constant, thence is described an LTI identification algorithm to be used to estimate the cell model in each segment. A Randles circuit is introduced to the model to describe the diffusion process. This model includes the so called Warburg impedance which is as fractional system. This impedance is discussed and it is approximatted by a finite order linear time invariant state-space model. Also, after presenting the simplified Randles circuit, is stated an identification algorithm that estimates the parameters of this model. The Th\'evenin model is presented as an alternative to the Randles circuit. An algorithm to identify a Th\'evenin model of 1st and 2nd order is enunciated. The performances of the simplified randles model and of the two Th\'evenin models models described and its respective identification algorithms, are discussed and compared using an experimental set of data.

==> bodeMag-table.tex <==
\draw[red,thick] plot coordinates{
(-3,25.0434)
(-2.9697,24.7372)
(-2.93939,24.4298)
(-2.90909,24.1217)
(-2.87879,23.8132)
(-2.84848,23.5051)
(-2.81818,23.1977)
(-2.78788,22.8915)
(-2.75758,22.5868)
(-2.72727,22.2839)
(-2.69697,21.9827)
(-2.66667,21.6831)
(-2.63636,21.3848)
(-2.60606,21.0875)
(-2.57576,20.7906)
(-2.54545,20.4937)
(-2.51515,20.196)
(-2.48485,19.8972)
(-2.45455,19.5969)
(-2.42424,19.2947)
(-2.39394,18.9906)
(-2.36364,18.6847)
(-2.33333,18.3771)
(-2.30303,18.0682)
(-2.27273,17.7585)
(-2.24242,17.4487)
(-2.21212,17.1393)
(-2.18182,16.8309)
(-2.15152,16.524)
(-2.12121,16.2191)
(-2.09091,15.9164)
(-2.06061,15.616)
(-2.0303,15.3179)
(-2,15.0216)
(-1.9697,14.727)
(-1.93939,14.4333)
(-1.90909,14.1399)
(-1.87879,13.8461)
(-1.84848,13.5514)
(-1.81818,13.2551)
(-1.78788,12.9567)
(-1.75758,12.656)
(-1.72727,12.3528)
(-1.69697,12.0473)
(-1.66667,11.7396)
(-1.63636,11.4303)
(-1.60606,11.1201)
(-1.57576,10.8095)
(-1.54545,10.4995)
(-1.51515,10.1908)
(-1.48485,9.88423)
(-1.45455,9.58035)
(-1.42424,9.2797)
(-1.39394,8.9826)
(-1.36364,8.68917)
(-1.33333,8.39931)
(-1.30303,8.11272)
(-1.27273,7.82893)
(-1.24242,7.54731)
(-1.21212,7.26712)
(-1.18182,6.98759)
(-1.15152,6.70796)
(-1.12121,6.42755)
(-1.09091,6.14577)
(-1.06061,5.86224)
(-1.0303,5.57677)
(-1,5.28941)
(-0.969697,5.00045)
(-0.939394,4.71042)
(-0.909091,4.42006)
(-0.878788,4.1303)
(-0.848485,3.84221)
(-0.818182,3.55694)
(-0.787879,3.27566)
(-0.757576,2.99953)
(-0.727273,2.72958)
(-0.69697,2.46675)
(-0.666667,2.21175)
(-0.636364,1.96512)
(-0.606061,1.72713)
(-0.575758,1.49785)
(-0.545455,1.27713)
(-0.515152,1.06461)
(-0.484848,0.859778)
(-0.454545,0.662009)
(-0.424242,0.470629)
(-0.393939,0.284973)
(-0.363636,0.104458)
(-0.333333,-0.0713403)
(-0.30303,-0.242607)
(-0.272727,-0.409204)
(-0.242424,-0.570582)
(-0.212121,-0.72569)
(-0.181818,-0.87289)
(-0.151515,-1.00986)
(-0.121212,-1.1335)
(-0.0909091,-1.23984)
(-0.0606061,-1.32394)
(-0.030303,-1.3798)
(0,-1.40023)
};

==> bodeMagC-Table.tex <==
\draw[thick,red] plot coordinates{
(-6,45.2559)
(-5.99199,45.2559)
(-5.98398,45.2558)
(-5.97598,45.2558)
(-5.96797,45.2557)
(-5.95996,45.2556)
(-5.95195,45.2556)
(-5.94394,45.2555)
(-5.93594,45.2555)
(-5.92793,45.2554)
(-5.91992,45.2553)
(-5.91191,45.2553)
(-5.9039,45.2552)
(-5.8959,45.2551)
(-5.88789,45.255)
(-5.87988,45.255)
(-5.87187,45.2549)
(-5.86386,45.2548)
(-5.85586,45.2547)
(-5.84785,45.2546)
(-5.83984,45.2545)
(-5.83183,45.2544)
(-5.82382,45.2543)
(-5.81582,45.2542)
(-5.80781,45.2541)
(-5.7998,45.254)
(-5.79179,45.2538)
(-5.78378,45.2537)
(-5.77578,45.2536)
(-5.76777,45.2535)
(-5.75976,45.2533)
(-5.75175,45.2532)
(-5.74374,45.253)
(-5.73574,45.2529)
(-5.72773,45.2527)
(-5.71972,45.2525)
(-5.71171,45.2524)
(-5.7037,45.2522)
(-5.6957,45.252)
(-5.68769,45.2518)
(-5.67968,45.2516)
(-5.67167,45.2514)
(-5.66366,45.2512)
(-5.65566,45.2509)
(-5.64765,45.2507)
(-5.63964,45.2505)
(-5.63163,45.2502)
(-5.62362,45.2499)
(-5.61562,45.2497)
(-5.60761,45.2494)
(-5.5996,45.2491)
(-5.59159,45.2488)
(-5.58358,45.2485)
(-5.57558,45.2481)
(-5.56757,45.2478)
(-5.55956,45.2475)
(-5.55155,45.2471)
(-5.54354,45.2467)
(-5.53554,45.2463)
(-5.52753,45.2459)
(-5.51952,45.2455)
(-5.51151,45.2451)
(-5.5035,45.2446)
(-5.4955,45.2441)
(-5.48749,45.2436)
(-5.47948,45.2431)
(-5.47147,45.2426)
(-5.46346,45.2421)
(-5.45546,45.2415)
(-5.44745,45.2409)
(-5.43944,45.2403)
(-5.43143,45.2397)
(-5.42342,45.239)
(-5.41542,45.2383)
(-5.40741,45.2376)
(-5.3994,45.2369)
(-5.39139,45.2361)
(-5.38338,45.2353)
(-5.37538,45.2345)
(-5.36737,45.2337)
(-5.35936,45.2328)
(-5.35135,45.2319)
(-5.34334,45.2309)
(-5.33534,45.2299)
(-5.32733,45.2289)
(-5.31932,45.2279)
(-5.31131,45.2268)
(-5.3033,45.2256)
(-5.2953,45.2244)
(-5.28729,45.2232)
(-5.27928,45.222)
(-5.27127,45.2206)
(-5.26326,45.2193)
(-5.25526,45.2179)
(-5.24725,45.2164)
(-5.23924,45.2149)
(-5.23123,45.2133)
(-5.22322,45.2116)
(-5.21522,45.2099)
(-5.20721,45.2082)
(-5.1992,45.2063)
(-5.19119,45.2044)
(-5.18318,45.2025)
(-5.17518,45.2004)
(-5.16717,45.1983)
(-5.15916,45.1961)
(-5.15115,45.1939)
(-5.14314,45.1915)
(-5.13514,45.189)
(-5.12713,45.1865)
(-5.11912,45.1839)
(-5.11111,45.1812)
(-5.1031,45.1783)
(-5.0951,45.1754)
(-5.08709,45.1724)
(-5.07908,45.1692)
(-5.07107,45.1659)
(-5.06306,45.1626)
(-5.05506,45.159)
(-5.04705,45.1554)
(-5.03904,45.1516)
(-5.03103,45.1477)
(-5.02302,45.1437)
(-5.01502,45.1395)
(-5.00701,45.1351)
(-4.999,45.1306)
(-4.99099,45.1259)
(-4.98298,45.1211)
(-4.97497,45.1161)
(-4.96697,45.1108)
(-4.95896,45.1055)
(-4.95095,45.0999)
(-4.94294,45.0941)
(-4.93493,45.0881)
(-4.92693,45.0819)
(-4.91892,45.0754)
(-4.91091,45.0688)
(-4.9029,45.0619)
(-4.89489,45.0547)
(-4.88689,45.0473)
(-4.87888,45.0396)
(-4.87087,45.0317)
(-4.86286,45.0235)
(-4.85485,45.015)
(-4.84685,45.0062)
(-4.83884,44.997)
(-4.83083,44.9876)
(-4.82282,44.9778)
(-4.81481,44.9677)
(-4.80681,44.9572)
(-4.7988,44.9464)
(-4.79079,44.9352)
(-4.78278,44.9236)
(-4.77477,44.9116)
(-4.76677,44.8992)
(-4.75876,44.8864)
(-4.75075,44.8731)
(-4.74274,44.8594)
(-4.73473,44.8452)
(-4.72673,44.8306)
(-4.71872,44.8154)
(-4.71071,44.7997)
(-4.7027,44.7836)
(-4.69469,44.7669)
(-4.68669,44.7496)
(-4.67868,44.7317)
(-4.67067,44.7133)
(-4.66266,44.6943)
(-4.65465,44.6747)
(-4.64665,44.6544)
(-4.63864,44.6335)
(-4.63063,44.6119)
(-4.62262,44.5896)
(-4.61461,44.5667)
(-4.60661,44.543)
(-4.5986,44.5185)
(-4.59059,44.4934)
(-4.58258,44.4674)
(-4.57457,44.4407)
(-4.56657,44.4131)
(-4.55856,44.3847)
(-4.55055,44.3555)
(-4.54254,44.3254)
(-4.53453,44.2944)
(-4.52653,44.2625)
(-4.51852,44.2298)
(-4.51051,44.196)
(-4.5025,44.1613)
(-4.49449,44.1257)
(-4.48649,44.089)
(-4.47848,44.0514)
(-4.47047,44.0127)
(-4.46246,43.973)
(-4.45445,43.9322)
(-4.44645,43.8903)
(-4.43844,43.8474)
(-4.43043,43.8033)
(-4.42242,43.7582)
(-4.41441,43.7119)
(-4.40641,43.6644)
(-4.3984,43.6159)
(-4.39039,43.5661)
(-4.38238,43.5152)
(-4.37437,43.463)
(-4.36637,43.4097)
(-4.35836,43.3552)
(-4.35035,43.2994)
(-4.34234,43.2424)
(-4.33433,43.1842)
(-4.32633,43.1248)
(-4.31832,43.0641)
(-4.31031,43.0022)
(-4.3023,42.9391)
(-4.29429,42.8747)
(-4.28629,42.809)
(-4.27828,42.7422)
(-4.27027,42.6741)
(-4.26226,42.6047)
(-4.25425,42.5342)
(-4.24625,42.4624)
(-4.24622,42.4621)
(-4.23824,42.3894)
(-4.23023,42.3152)
(-4.22222,42.2398)
(-4.21421,42.1633)
(-4.20621,42.0855)
(-4.1982,42.0067)
(-4.19019,41.9266)
(-4.18218,41.8455)
(-4.17417,41.7633)
(-4.16617,41.68)
(-4.15816,41.5956)
(-4.15015,41.5101)
(-4.14214,41.4237)
(-4.13413,41.3362)
(-4.12613,41.2478)
(-4.11812,41.1585)
(-4.11011,41.0682)
(-4.1021,40.977)
(-4.09409,40.885)
(-4.08609,40.7921)
(-4.07808,40.6984)
(-4.07007,40.604)
(-4.06206,40.5088)
(-4.05405,40.4129)
(-4.04605,40.3163)
(-4.03804,40.219)
(-4.03003,40.1212)
(-4.02202,40.0228)
(-4.01401,39.9238)
(-4.00601,39.8243)
(-3.998,39.7244)
(-3.98999,39.624)
(-3.98198,39.5232)
(-3.97397,39.4221)
(-3.96597,39.3206)
(-3.95796,39.2189)
(-3.94995,39.1168)
(-3.94194,39.0146)
(-3.93393,38.9122)
(-3.92593,38.8096)
(-3.91792,38.707)
(-3.90991,38.6042)
(-3.9019,38.5014)
(-3.89389,38.3987)
(-3.88589,38.2959)
(-3.87788,38.1932)
(-3.86987,38.0906)
(-3.86186,37.9882)
(-3.85385,37.8859)
(-3.84585,37.7838)
(-3.83784,37.6819)
(-3.82983,37.5803)
(-3.82182,37.479)
(-3.81381,37.378)
(-3.80581,37.2774)
(-3.7978,37.1771)
(-3.78979,37.0772)
(-3.78178,36.9777)
(-3.77377,36.8787)
(-3.76577,36.7802)
(-3.75776,36.6821)
(-3.74975,36.5845)
(-3.74174,36.4875)
(-3.73373,36.391)
(-3.72573,36.2951)
(-3.71772,36.1997)
(-3.70971,36.105)
(-3.7017,36.0108)
(-3.69369,35.9173)
(-3.68569,35.8243)
(-3.67768,35.732)
(-3.66967,35.6404)
(-3.66166,35.5493)
(-3.65365,35.4589)
(-3.64565,35.3692)
(-3.63764,35.2801)
(-3.62963,35.1916)
(-3.62939,35.189)
(-3.62162,35.1038)
(-3.61361,35.0166)
(-3.60561,34.9301)
(-3.5976,34.8442)
(-3.58959,34.7589)
(-3.58158,34.6742)
(-3.57357,34.59)
(-3.56557,34.5065)
(-3.55756,34.4236)
(-3.54955,34.3412)
(-3.54154,34.2593)
(-3.53353,34.178)
(-3.52553,34.0971)
(-3.51752,34.0168)
(-3.50951,33.9369)
(-3.5015,33.8575)
(-3.49349,33.7785)
(-3.48549,33.6999)
(-3.47748,33.6217)
(-3.46947,33.5438)
(-3.46146,33.4663)
(-3.45345,33.389)
(-3.44545,33.3121)
(-3.43744,33.2354)
(-3.42943,33.159)
(-3.42142,33.0828)
(-3.41341,33.0068)
(-3.40541,32.9309)
(-3.3974,32.8552)
(-3.38939,32.7795)
(-3.38138,32.704)
(-3.37337,32.6286)
(-3.36537,32.5532)
(-3.35736,32.4778)
(-3.34935,32.4024)
(-3.34134,32.327)
(-3.33333,32.2515)
(-3.32533,32.176)
(-3.31732,32.1004)
(-3.30931,32.0248)
(-3.3013,31.949)
(-3.29329,31.873)
(-3.28529,31.797)
(-3.27728,31.7207)
(-3.26927,31.6443)
(-3.26126,31.5677)
(-3.25325,31.4909)
(-3.24525,31.414)
(-3.23724,31.3368)
(-3.22923,31.2594)
(-3.22122,31.1817)
(-3.21534,31.1246)
(-3.21321,31.1039)
(-3.20521,31.0258)
(-3.1972,30.9475)
(-3.18919,30.8689)
(-3.18118,30.7901)
(-3.17317,30.7111)
(-3.16517,30.6319)
(-3.15716,30.5524)
(-3.14915,30.4727)
(-3.14114,30.3928)
(-3.13313,30.3127)
(-3.12513,30.2324)
(-3.11712,30.1519)
(-3.10911,30.0713)
(-3.1011,29.9904)
(-3.09309,29.9094)
(-3.08509,29.8283)
(-3.07708,29.747)
(-3.06907,29.6656)
(-3.06106,29.5841)
(-3.05305,29.5025)
(-3.04505,29.4208)
(-3.03704,29.339)
(-3.02903,29.2572)
(-3.02102,29.1753)
(-3.01301,29.0934)
(-3.00501,29.0115)
(-2.997,28.9296)
(-2.98899,28.8477)
(-2.98098,28.7658)
(-2.97297,28.684)
(-2.96496,28.6022)
(-2.95696,28.5204)
(-2.94895,28.4387)
(-2.94094,28.3571)
(-2.93293,28.2756)
(-2.92492,28.1942)
(-2.91692,28.1129)
(-2.90891,28.0316)
(-2.9009,27.9505)
(-2.89289,27.8696)
(-2.88488,27.7887)
(-2.87688,27.708)
(-2.87185,27.6574)
(-2.86887,27.6274)
(-2.86086,27.5469)
(-2.85285,27.4666)
(-2.84484,27.3863)
(-2.83684,27.3063)
(-2.82883,27.2263)
(-2.82082,27.1465)
(-2.81281,27.0668)
(-2.8048,26.9872)
(-2.7968,26.9078)
(-2.78879,26.8284)
(-2.78078,26.7491)
(-2.77277,26.67)
(-2.76476,26.5909)
(-2.75676,26.5119)
(-2.74875,26.4329)
(-2.74074,26.3541)
(-2.73273,26.2752)
(-2.72472,26.1965)
(-2.71672,26.1177)
(-2.70871,26.039)
(-2.7007,25.9602)
(-2.69269,25.8815)
(-2.68468,25.8028)
(-2.67668,25.724)
(-2.66867,25.6453)
(-2.66066,25.5664)
(-2.65265,25.4876)
(-2.64464,25.4086)
(-2.63664,25.3296)
(-2.62863,25.2506)
(-2.62062,25.1714)
(-2.61261,25.0922)
(-2.6046,25.0129)
(-2.5966,24.9335)
(-2.58859,24.8539)
(-2.58058,24.7743)
(-2.57257,24.6946)
(-2.56456,24.6147)
(-2.55656,24.5347)
(-2.5526,24.4951)
(-2.54855,24.4546)
(-2.54054,24.3744)
(-2.53253,24.2941)
(-2.52452,24.2137)
(-2.51652,24.1331)
(-2.50851,24.0524)
(-2.5005,23.9717)
(-2.49249,23.8908)
(-2.48448,23.8098)
(-2.47648,23.7288)
(-2.46847,23.6476)
(-2.46046,23.5664)
(-2.45245,23.4851)
(-2.44444,23.4037)
(-2.43644,23.3223)
(-2.42843,23.2409)
(-2.42042,23.1594)
(-2.41241,23.0779)
(-2.4044,22.9963)
(-2.3964,22.9148)
(-2.38839,22.8332)
(-2.38038,22.7517)
(-2.37237,22.6702)
(-2.36436,22.5887)
(-2.35636,22.5073)
(-2.34835,22.4259)
(-2.34034,22.3445)
(-2.33233,22.2633)
(-2.32432,22.1821)
(-2.31632,22.1009)
(-2.30831,22.0199)
(-2.3003,21.939)
(-2.29229,21.8582)
(-2.28428,21.7775)
(-2.27628,21.6968)
(-2.26827,21.6164)
(-2.26026,21.536)
(-2.25225,21.4557)
(-2.24424,21.3756)
(-2.23711,21.3043)
(-2.23624,21.2956)
(-2.22823,21.2157)
(-2.22022,21.136)
(-2.21221,21.0563)
(-2.2042,20.9768)
(-2.1962,20.8974)
(-2.18819,20.8181)
(-2.18018,20.7389)
(-2.17217,20.6599)
(-2.16416,20.5809)
(-2.15616,20.502)
(-2.14815,20.4232)
(-2.14014,20.3444)
(-2.13213,20.2658)
(-2.12412,20.1872)
(-2.11612,20.1086)
(-2.10811,20.0301)
(-2.1001,19.9516)
(-2.09209,19.8731)
(-2.08408,19.7947)
(-2.07608,19.7162)
(-2.06807,19.6377)
(-2.06006,19.5592)
(-2.05205,19.4807)
(-2.04404,19.4021)
(-2.03604,19.3235)
(-2.02803,19.2448)
(-2.02002,19.1661)
(-2.01201,19.0872)
(-2.004,19.0083)
(-1.996,18.9293)
(-1.98799,18.8502)
(-1.97998,18.7709)
(-1.97197,18.6916)
(-1.96396,18.6121)
(-1.95596,18.5325)
(-1.94795,18.4528)
(-1.93994,18.3729)
(-1.93193,18.293)
(-1.92392,18.2128)
(-1.91747,18.1482)
(-1.91592,18.1326)
(-1.90791,18.0522)
(-1.8999,17.9716)
(-1.89189,17.891)
(-1.88388,17.8102)
(-1.87588,17.7292)
(-1.86787,17.6482)
(-1.85986,17.567)
(-1.85185,17.4857)
(-1.84384,17.4043)
(-1.83584,17.3228)
(-1.82783,17.2413)
(-1.81982,17.1596)
(-1.81181,17.0779)
(-1.8038,16.9961)
(-1.7958,16.9142)
(-1.78779,16.8323)
(-1.77978,16.7504)
(-1.77177,16.6685)
(-1.76376,16.5865)
(-1.75576,16.5045)
(-1.74775,16.4226)
(-1.73974,16.3407)
(-1.73173,16.2588)
(-1.72372,16.177)
(-1.71572,16.0952)
(-1.70771,16.0135)
(-1.6997,15.9318)
(-1.69169,15.8503)
(-1.68368,15.7689)
(-1.67568,15.6875)
(-1.66767,15.6063)
(-1.65966,15.5252)
(-1.65165,15.4442)
(-1.64364,15.3634)
(-1.63564,15.2827)
(-1.62763,15.2022)
(-1.61962,15.1218)
(-1.61161,15.0416)
(-1.6036,14.9615)
(-1.5956,14.8816)
(-1.58953,14.8211)
(-1.58759,14.8018)
(-1.57958,14.7222)
(-1.57157,14.6428)
(-1.56356,14.5635)
(-1.55556,14.4844)
(-1.54755,14.4054)
(-1.53954,14.3266)
(-1.53153,14.2479)
(-1.52352,14.1693)
(-1.51552,14.0909)
(-1.50751,14.0125)
(-1.4995,13.9343)
(-1.49149,13.8562)
(-1.48348,13.7782)
(-1.47548,13.7002)
(-1.46747,13.6224)
(-1.45946,13.5445)
(-1.45145,13.4668)
(-1.44344,13.389)
(-1.43544,13.3113)
(-1.42743,13.2336)
(-1.41942,13.1559)
(-1.41141,13.0781)
(-1.4034,13.0004)
(-1.3954,12.9225)
(-1.38739,12.8447)
(-1.37938,12.7667)
(-1.37137,12.6887)
(-1.36336,12.6106)
(-1.35536,12.5324)
(-1.34735,12.4541)
(-1.33934,12.3756)
(-1.33133,12.2971)
(-1.32332,12.2183)
(-1.31532,12.1395)
(-1.30731,12.0605)
(-1.2993,11.9813)
(-1.29129,11.9019)
(-1.28328,11.8224)
(-1.27528,11.7427)
(-1.26727,11.6628)
(-1.25926,11.5827)
(-1.25125,11.5025)
(-1.25031,11.4931)
(-1.24324,11.4221)
(-1.23524,11.3414)
(-1.22723,11.2607)
(-1.21922,11.1797)
(-1.21121,11.0986)
(-1.2032,11.0173)
(-1.1952,10.9358)
(-1.18719,10.8542)
(-1.17918,10.7724)
(-1.17117,10.6905)
(-1.16316,10.6085)
(-1.15516,10.5263)
(-1.14715,10.4441)
(-1.13914,10.3617)
(-1.13113,10.2793)
(-1.12312,10.1968)
(-1.11512,10.1142)
(-1.10711,10.0316)
(-1.0991,9.94896)
(-1.09109,9.86631)
(-1.08308,9.78365)
(-1.07508,9.70101)
(-1.06707,9.6184)
(-1.05906,9.53583)
(-1.05105,9.45331)
(-1.04304,9.37087)
(-1.03504,9.28851)
(-1.02703,9.20625)
(-1.01902,9.1241)
(-1.01101,9.04208)
(-1.003,8.9602)
(-0.994995,8.87847)
(-0.986987,8.7969)
(-0.978979,8.7155)
(-0.970971,8.63429)
(-0.962963,8.55326)
(-0.954955,8.47244)
(-0.946947,8.39183)
(-0.938939,8.31142)
(-0.930931,8.23124)
(-0.922923,8.15129)
(-0.914915,8.07156)
(-0.906907,7.99206)
(-0.898899,7.91279)
(-0.898272,7.90659)
(-0.890891,7.83375)
(-0.882883,7.75494)
(-0.874875,7.67637)
(-0.866867,7.59802)
(-0.858859,7.51989)
(-0.850851,7.44198)
(-0.842843,7.36429)
(-0.834835,7.28679)
(-0.826827,7.2095)
(-0.818819,7.13239)
(-0.810811,7.05546)
(-0.802803,6.9787)
(-0.794795,6.9021)
(-0.786787,6.82564)
(-0.778779,6.74932)
(-0.770771,6.67311)
(-0.762763,6.597)
(-0.754755,6.52099)
(-0.746747,6.44505)
(-0.738739,6.36918)
(-0.730731,6.29334)
(-0.722723,6.21754)
(-0.714715,6.14175)
(-0.706707,6.06596)
(-0.698699,5.99015)
(-0.690691,5.9143)
(-0.682683,5.83841)
(-0.674675,5.76244)
(-0.666667,5.6864)
(-0.658659,5.61027)
(-0.650651,5.53403)
(-0.642643,5.45766)
(-0.634635,5.38116)
(-0.626627,5.30451)
(-0.618619,5.2277)
(-0.610611,5.15072)
(-0.602603,5.07357)
(-0.594595,4.99622)
(-0.586587,4.91868)
(-0.578579,4.84093)
(-0.570571,4.76298)
(-0.562563,4.68481)
(-0.554555,4.60642)
(-0.546547,4.52781)
(-0.538539,4.44898)
(-0.530531,4.36992)
(-0.52875,4.35231)
(-0.522523,4.29065)
(-0.514515,4.21115)
(-0.506507,4.13144)
(-0.498498,4.05152)
(-0.49049,3.97139)
(-0.482482,3.89106)
(-0.474474,3.81054)
(-0.466466,3.72983)
(-0.458458,3.64896)
(-0.45045,3.56792)
(-0.442442,3.48674)
(-0.434434,3.40542)
(-0.426426,3.32397)
(-0.418418,3.24243)
(-0.41041,3.16079)
(-0.402402,3.07908)
(-0.394394,2.99731)
(-0.386386,2.9155)
(-0.378378,2.83367)
(-0.37037,2.75184)
(-0.362362,2.67003)
(-0.354354,2.58825)
(-0.346346,2.50653)
(-0.338338,2.42489)
(-0.33033,2.34334)
(-0.322322,2.26192)
(-0.314314,2.18063)
(-0.306306,2.09949)
(-0.298298,2.01854)
(-0.29029,1.93778)
(-0.282282,1.85723)
(-0.274274,1.77692)
(-0.266266,1.69686)
(-0.258258,1.61706)
(-0.25025,1.53756)
(-0.242242,1.45835)
(-0.234234,1.37946)
(-0.226226,1.3009)
(-0.218218,1.22267)
(-0.21021,1.14481)
(-0.202202,1.06731)
(-0.194194,0.990181)
(-0.186186,0.913438)
(-0.178178,0.837085)
(-0.17017,0.761128)
(-0.162162,0.685572)
(-0.154154,0.610419)
(-0.147558,0.548817)
(-0.146146,0.535673)
(-0.138138,0.461333)
(-0.13013,0.387397)
(-0.122122,0.313865)
(-0.114114,0.240731)
(-0.106106,0.167991)
(-0.0980981,0.0956376)
(-0.0900901,0.0236622)
(-0.0820821,-0.0479448)
(-0.0740741,-0.119195)
(-0.0660661,-0.1901)
(-0.0580581,-0.260674)
(-0.0500501,-0.330934)
(-0.042042,-0.400895)
(-0.034034,-0.470576)
(-0.026026,-0.539996)
(-0.018018,-0.609176)
(-0.01001,-0.678138)
(-0.002002,-0.746905)
(0.00600601,-0.8155)
(0.014014,-0.88395)
(0.022022,-0.95228)
(0.03003,-1.02052)
(0.038038,-1.08869)
(0.046046,-1.15683)
(0.0540541,-1.22496)
(0.0620621,-1.29312)
(0.0700701,-1.36133)
(0.0780781,-1.42964)
(0.0860861,-1.49806)
(0.0940941,-1.56663)
(0.102102,-1.63539)
(0.11011,-1.70437)
(0.118118,-1.7736)
(0.126126,-1.84312)
(0.134134,-1.91296)
(0.142142,-1.98316)
(0.15015,-2.05374)
(0.158158,-2.12474)
(0.166166,-2.19621)
(0.174174,-2.26816)
(0.182182,-2.34063)
(0.19019,-2.41367)
(0.198198,-2.48729)
(0.206206,-2.56153)
(0.214214,-2.63642)
(0.222222,-2.712)
(0.23023,-2.78828)
(0.238238,-2.86531)
(0.246246,-2.94312)
(0.254254,-3.02172)
(0.262262,-3.10114)
(0.27027,-3.18142)
(0.278278,-3.26257)
(0.286286,-3.34463)
(0.294294,-3.42761)
(0.302302,-3.51154)
(0.31031,-3.59643)
(0.318318,-3.68231)
(0.326326,-3.7692)
(0.334334,-3.8571)
(0.342342,-3.94605)
(0.35035,-4.03605)
(0.358358,-4.12712)
(0.360731,-4.15431)
(0.366366,-4.21927)
(0.374374,-4.31251)
(0.382382,-4.40685)
(0.39039,-4.5023)
(0.398398,-4.59887)
(0.406406,-4.69656)
(0.414414,-4.79539)
(0.422422,-4.89534)
(0.43043,-4.99643)
(0.438438,-5.09866)
(0.446446,-5.20203)
(0.454454,-5.30654)
(0.462462,-5.41218)
(0.47047,-5.51895)
(0.478478,-5.62685)
(0.486486,-5.73588)
(0.494494,-5.84602)
(0.502503,-5.95728)
(0.510511,-6.06964)
(0.518519,-6.18309)
(0.526527,-6.29763)
(0.534535,-6.41325)
(0.542543,-6.52993)
(0.550551,-6.64767)
(0.558559,-6.76645)
(0.566567,-6.88625)
(0.574575,-7.00708)
(0.582583,-7.1289)
(0.590591,-7.25172)
(0.598599,-7.3755)
(0.606607,-7.50025)
(0.614615,-7.62593)
(0.622623,-7.75255)
(0.630631,-7.88008)
(0.638639,-8.0085)
(0.646647,-8.1378)
(0.654655,-8.26796)
(0.662663,-8.39896)
(0.670671,-8.5308)
(0.678679,-8.66344)
(0.686687,-8.79688)
(0.694695,-8.9311)
(0.702703,-9.06608)
(0.710711,-9.2018)
(0.718719,-9.33825)
(0.726727,-9.4754)
(0.734735,-9.61325)
(0.742743,-9.75178)
(0.750751,-9.89096)
(0.758759,-10.0308)
(0.766767,-10.1712)
(0.774775,-10.3123)
(0.782783,-10.454)
(0.790791,-10.5962)
(0.798799,-10.739)
(0.806807,-10.8824)
(0.814815,-11.0263)
(0.822823,-11.1707)
(0.830831,-11.3156)
(0.838839,-11.461)
(0.846847,-11.6069)
(0.854855,-11.7532)
(0.862863,-11.9)
(0.870871,-12.0473)
(0.878879,-12.1949)
(0.886887,-12.343)
(0.894895,-12.4915)
(0.902903,-12.6403)
(0.910911,-12.7896)
(0.918919,-12.9392)
(0.926927,-13.0891)
(0.934935,-13.2394)
(0.942943,-13.39)
(0.950951,-13.541)
(0.958959,-13.6922)
(0.966967,-13.8438)
(0.974975,-13.9957)
(0.982983,-14.1478)
(0.990991,-14.3002)
(0.998999,-14.4529)
(1.00701,-14.6058)
(1.01502,-14.759)
(1.02302,-14.9124)
(1.03103,-15.0661)
(1.03904,-15.2199)
(1.04705,-15.374)
(1.05506,-15.5283)
(1.06306,-15.6829)
(1.07107,-15.8376)
(1.07908,-15.9925)
(1.08709,-16.1475)
(1.0951,-16.3028)
(1.1031,-16.4582)
(1.11111,-16.6138)
(1.11912,-16.7696)
(1.12713,-16.9255)
(1.13514,-17.0815)
(1.14314,-17.2377)
(1.15115,-17.3941)
(1.15916,-17.5505)
(1.16717,-17.7071)
(1.17518,-17.8639)
(1.18318,-18.0207)
(1.19119,-18.1777)
(1.1992,-18.3348)
(1.20721,-18.492)
(1.21522,-18.6493)
(1.22322,-18.8066)
(1.23123,-18.9641)
(1.23924,-19.1217)
(1.24725,-19.2794)
(1.25526,-19.4372)
(1.26326,-19.595)
(1.27127,-19.753)
(1.27928,-19.911)
(1.28729,-20.0691)
(1.2953,-20.2272)
(1.3033,-20.3855)
(1.31131,-20.5438)
(1.31932,-20.7022)
(1.32733,-20.8606)
(1.33534,-21.0191)
(1.34334,-21.1777)
(1.35135,-21.3363)
(1.35936,-21.4949)
(1.36737,-21.6537)
(1.37538,-21.8124)
(1.38338,-21.9713)
(1.39139,-22.1301)
(1.3994,-22.289)
(1.40741,-22.448)
(1.41542,-22.607)
(1.42342,-22.7661)
(1.43143,-22.9252)
(1.43944,-23.0843)
(1.44745,-23.2434)
(1.45546,-23.4026)
(1.46346,-23.5619)
(1.47147,-23.7211)
(1.47948,-23.8804)
(1.48749,-24.0398)
(1.4955,-24.1991)
(1.5035,-24.3585)
(1.51151,-24.5179)
(1.51952,-24.6774)
(1.52753,-24.8368)
(1.53554,-24.9963)
(1.54354,-25.1559)
(1.55155,-25.3154)
(1.55956,-25.475)
(1.56757,-25.6345)
(1.57558,-25.7942)
(1.58358,-25.9538)
(1.59159,-26.1134)
(1.5996,-26.2731)
(1.60761,-26.4328)
(1.61562,-26.5925)
(1.62362,-26.7522)
(1.63163,-26.9119)
(1.63964,-27.0717)
(1.64765,-27.2314)
(1.65566,-27.3912)
(1.66366,-27.551)
(1.67167,-27.7108)
(1.67968,-27.8706)
(1.68769,-28.0304)
(1.6957,-28.1903)
(1.7037,-28.3501)
(1.71171,-28.51)
(1.71972,-28.6699)
(1.72773,-28.8298)
(1.73574,-28.9896)
(1.74374,-29.1496)
(1.75175,-29.3095)
(1.75976,-29.4694)
(1.76777,-29.6293)
(1.77578,-29.7893)
(1.78378,-29.9492)
(1.79179,-30.1092)
(1.7998,-30.2691)
(1.80781,-30.4291)
(1.81582,-30.5891)
(1.82382,-30.749)
(1.83183,-30.909)
(1.83984,-31.069)
(1.84785,-31.229)
(1.85586,-31.389)
(1.86386,-31.5491)
(1.87187,-31.7091)
(1.87988,-31.8691)
(1.88789,-32.0291)
(1.8959,-32.1892)
(1.9039,-32.3492)
(1.91191,-32.5092)
(1.91992,-32.6693)
(1.92793,-32.8293)
(1.93594,-32.9894)
(1.94394,-33.1494)
(1.95195,-33.3095)
(1.95996,-33.4696)
(1.96797,-33.6296)
(1.97598,-33.7897)
(1.98398,-33.9498)
(1.99199,-34.1099)
(2,-34.2699)
};

==> bodePhase-table.tex <==
\draw[red,thick] plot coordinates{
(-3,-11.2864)
(-2.9697,-11.2951)
(-2.93939,-11.3019)
(-2.90909,-11.3064)
(-2.87879,-11.3083)
(-2.84848,-11.3076)
(-2.81818,-11.3045)
(-2.78788,-11.2996)
(-2.75758,-11.2935)
(-2.72727,-11.2871)
(-2.69697,-11.2812)
(-2.66667,-11.2768)
(-2.63636,-11.2746)
(-2.60606,-11.2752)
(-2.57576,-11.279)
(-2.54545,-11.2861)
(-2.51515,-11.2965)
(-2.48485,-11.3096)
(-2.45455,-11.3249)
(-2.42424,-11.3416)
(-2.39394,-11.3588)
(-2.36364,-11.3756)
(-2.33333,-11.391)
(-2.30303,-11.4044)
(-2.27273,-11.4153)
(-2.24242,-11.4235)
(-2.21212,-11.4289)
(-2.18182,-11.4319)
(-2.15152,-11.4331)
(-2.12121,-11.4334)
(-2.09091,-11.4338)
(-2.06061,-11.4354)
(-2.0303,-11.4394)
(-2,-11.4467)
(-1.9697,-11.4584)
(-1.93939,-11.475)
(-1.90909,-11.4971)
(-1.87879,-11.5247)
(-1.84848,-11.5577)
(-1.81818,-11.5955)
(-1.78788,-11.6374)
(-1.75758,-11.6826)
(-1.72727,-11.7301)
(-1.69697,-11.7787)
(-1.66667,-11.8276)
(-1.63636,-11.876)
(-1.60606,-11.9233)
(-1.57576,-11.9693)
(-1.54545,-12.0141)
(-1.51515,-12.0583)
(-1.48485,-12.1026)
(-1.45455,-12.1482)
(-1.42424,-12.1965)
(-1.39394,-12.2492)
(-1.36364,-12.308)
(-1.33333,-12.3748)
(-1.30303,-12.4512)
(-1.27273,-12.5389)
(-1.24242,-12.6392)
(-1.21212,-12.7531)
(-1.18182,-12.8815)
(-1.15152,-13.0249)
(-1.12121,-13.1834)
(-1.09091,-13.3569)
(-1.06061,-13.5452)
(-1.0303,-13.7478)
(-1,-13.9644)
(-0.969697,-14.1947)
(-0.939394,-14.4386)
(-0.909091,-14.6963)
(-0.878788,-14.9682)
(-0.848485,-15.2556)
(-0.818182,-15.5598)
(-0.787879,-15.883)
(-0.757576,-16.2279)
(-0.727273,-16.5975)
(-0.69697,-16.9956)
(-0.666667,-17.4261)
(-0.636364,-17.8937)
(-0.606061,-18.4029)
(-0.575758,-18.9587)
(-0.545455,-19.5662)
(-0.515152,-20.2305)
(-0.484848,-20.9566)
(-0.454545,-21.7495)
(-0.424242,-22.6141)
(-0.393939,-23.5553)
(-0.363636,-24.5775)
(-0.333333,-25.6855)
(-0.30303,-26.8837)
(-0.272727,-28.1766)
(-0.242424,-29.569)
(-0.212121,-31.0655)
(-0.181818,-32.6716)
(-0.151515,-34.393)
(-0.121212,-36.2363)
(-0.0909091,-38.2091)
(-0.0606061,-40.3201)
(-0.030303,-42.5797)
(0,-45)
};

==> bodePhaseC-Table.tex <==
\draw[thick,red] plot coordinates{
(-6,-60.8311)
(-5.99199,-60.8465)
(-5.98398,-60.8623)
(-5.97598,-60.8783)
(-5.96797,-60.8947)
(-5.95996,-60.9113)
(-5.95195,-60.9283)
(-5.94394,-60.9455)
(-5.93594,-60.9631)
(-5.92793,-60.981)
(-5.91992,-60.9993)
(-5.91191,-61.0179)
(-5.9039,-61.0368)
(-5.8959,-61.0561)
(-5.88789,-61.0757)
(-5.87988,-61.0958)
(-5.87187,-61.1161)
(-5.86386,-61.1369)
(-5.85586,-61.1581)
(-5.84785,-61.1796)
(-5.83984,-61.2015)
(-5.83183,-61.2239)
(-5.82382,-61.2466)
(-5.81582,-61.2698)
(-5.80781,-61.2935)
(-5.7998,-61.3175)
(-5.79179,-61.342)
(-5.78378,-61.367)
(-5.77578,-61.3924)
(-5.76777,-61.4183)
(-5.75976,-61.4447)
(-5.75175,-61.4715)
(-5.74374,-61.4989)
(-5.73574,-61.5268)
(-5.72773,-61.5552)
(-5.71972,-61.5841)
(-5.71171,-61.6135)
(-5.7037,-61.6435)
(-5.6957,-61.6741)
(-5.68769,-61.7052)
(-5.67968,-61.7369)
(-5.67167,-61.7692)
(-5.66366,-61.8021)
(-5.65566,-61.8356)
(-5.64765,-61.8697)
(-5.63964,-61.9044)
(-5.63163,-61.9398)
(-5.62362,-61.9759)
(-5.61562,-62.0126)
(-5.60761,-62.05)
(-5.5996,-62.0881)
(-5.59159,-62.1269)
(-5.58358,-62.1664)
(-5.57558,-62.2066)
(-5.56757,-62.2476)
(-5.55956,-62.2894)
(-5.55155,-62.3319)
(-5.54354,-62.3752)
(-5.53554,-62.4193)
(-5.52753,-62.4643)
(-5.51952,-62.51)
(-5.51151,-62.5566)
(-5.5035,-62.6041)
(-5.4955,-62.6524)
(-5.48749,-62.7017)
(-5.47948,-62.7518)
(-5.47147,-62.8029)
(-5.46346,-62.8549)
(-5.45546,-62.9079)
(-5.44745,-62.9618)
(-5.43944,-63.0167)
(-5.43143,-63.0727)
(-5.42342,-63.1297)
(-5.41542,-63.1877)
(-5.40741,-63.2468)
(-5.3994,-63.307)
(-5.39139,-63.3683)
(-5.38338,-63.4307)
(-5.37538,-63.4943)
(-5.36737,-63.559)
(-5.35936,-63.6249)
(-5.35135,-63.6921)
(-5.34334,-63.7604)
(-5.33534,-63.8301)
(-5.32733,-63.901)
(-5.31932,-63.9731)
(-5.31131,-64.0466)
(-5.3033,-64.1215)
(-5.2953,-64.1977)
(-5.28729,-64.2753)
(-5.27928,-64.3544)
(-5.27127,-64.4348)
(-5.26326,-64.5168)
(-5.25526,-64.6002)
(-5.24725,-64.6851)
(-5.23924,-64.7716)
(-5.23123,-64.8597)
(-5.22322,-64.9493)
(-5.21522,-65.0406)
(-5.20721,-65.1335)
(-5.1992,-65.2281)
(-5.19119,-65.3244)
(-5.18318,-65.4225)
(-5.17518,-65.5223)
(-5.16717,-65.6239)
(-5.15916,-65.7274)
(-5.15115,-65.8326)
(-5.14314,-65.9398)
(-5.13514,-66.0489)
(-5.12713,-66.16)
(-5.11912,-66.273)
(-5.11111,-66.3881)
(-5.1031,-66.5051)
(-5.0951,-66.6243)
(-5.08709,-66.7456)
(-5.07908,-66.869)
(-5.07107,-66.9946)
(-5.06306,-67.1224)
(-5.05506,-67.2525)
(-5.04705,-67.3849)
(-5.03904,-67.5195)
(-5.03103,-67.6565)
(-5.02302,-67.796)
(-5.01502,-67.9378)
(-5.00701,-68.0821)
(-4.999,-68.2288)
(-4.99099,-68.3782)
(-4.98298,-68.53)
(-4.97497,-68.6845)
(-4.96697,-68.8416)
(-4.95896,-69.0014)
(-4.95095,-69.1639)
(-4.94294,-69.3292)
(-4.93493,-69.4972)
(-4.92693,-69.6681)
(-4.91892,-69.8418)
(-4.91091,-70.0184)
(-4.9029,-70.198)
(-4.89489,-70.3805)
(-4.88689,-70.566)
(-4.87888,-70.7545)
(-4.87087,-70.9461)
(-4.86286,-71.1408)
(-4.85485,-71.3386)
(-4.84685,-71.5396)
(-4.83884,-71.7439)
(-4.83083,-71.9513)
(-4.82282,-72.162)
(-4.81481,-72.376)
(-4.80681,-72.5933)
(-4.7988,-72.8139)
(-4.79079,-73.038)
(-4.78278,-73.2654)
(-4.77477,-73.4963)
(-4.76677,-73.7306)
(-4.75876,-73.9683)
(-4.75075,-74.2096)
(-4.74274,-74.4544)
(-4.73473,-74.7026)
(-4.72673,-74.9545)
(-4.71872,-75.2098)
(-4.71071,-75.4688)
(-4.7027,-75.7313)
(-4.69469,-75.9973)
(-4.68669,-76.267)
(-4.67868,-76.5402)
(-4.67067,-76.817)
(-4.66266,-77.0974)
(-4.65465,-77.3813)
(-4.64665,-77.6688)
(-4.63864,-77.9598)
(-4.63063,-78.2544)
(-4.62262,-78.5524)
(-4.61461,-78.854)
(-4.60661,-79.1589)
(-4.5986,-79.4673)
(-4.59059,-79.7791)
(-4.58258,-80.0942)
(-4.57457,-80.4126)
(-4.56657,-80.7342)
(-4.55856,-81.0591)
(-4.55055,-81.3871)
(-4.54254,-81.7181)
(-4.53453,-82.0522)
(-4.52653,-82.3891)
(-4.51852,-82.729)
(-4.51051,-83.0716)
(-4.5025,-83.4169)
(-4.49449,-83.7648)
(-4.48649,-84.1152)
(-4.47848,-84.468)
(-4.47047,-84.823)
(-4.46246,-85.1803)
(-4.45445,-85.5396)
(-4.44645,-85.9008)
(-4.43844,-86.2638)
(-4.43043,-86.6285)
(-4.42242,-86.9947)
(-4.41441,-87.3623)
(-4.40641,-87.7311)
(-4.3984,-88.101)
(-4.39039,-88.4719)
(-4.38238,-88.8434)
(-4.37437,-89.2156)
(-4.36637,-89.5882)
(-4.35836,-89.961)
(-4.35035,-90.3338)
(-4.34234,-90.7066)
(-4.33433,-91.079)
(-4.32633,-91.4509)
(-4.31832,-91.8221)
(-4.31031,-92.1924)
(-4.3023,-92.5616)
(-4.29429,-92.9295)
(-4.28629,-93.2959)
(-4.27828,-93.6606)
(-4.27027,-94.0234)
(-4.26226,-94.3841)
(-4.25425,-94.7424)
(-4.24625,-95.0982)
(-4.24622,-95.0995)
(-4.23824,-95.4512)
(-4.23023,-95.8014)
(-4.22222,-96.1483)
(-4.21421,-96.4919)
(-4.20621,-96.832)
(-4.1982,-97.1682)
(-4.19019,-97.5006)
(-4.18218,-97.8287)
(-4.17417,-98.1526)
(-4.16617,-98.4719)
(-4.15816,-98.7865)
(-4.15015,-99.0962)
(-4.14214,-99.4008)
(-4.13413,-99.7002)
(-4.12613,-99.9942)
(-4.11812,-100.283)
(-4.11011,-100.565)
(-4.1021,-100.842)
(-4.09409,-101.113)
(-4.08609,-101.378)
(-4.07808,-101.636)
(-4.07007,-101.888)
(-4.06206,-102.134)
(-4.05405,-102.373)
(-4.04605,-102.605)
(-4.03804,-102.83)
(-4.03003,-103.049)
(-4.02202,-103.26)
(-4.01401,-103.465)
(-4.00601,-103.662)
(-3.998,-103.853)
(-3.98999,-104.036)
(-3.98198,-104.212)
(-3.97397,-104.38)
(-3.96597,-104.542)
(-3.95796,-104.696)
(-3.94995,-104.843)
(-3.94194,-104.983)
(-3.93393,-105.115)
(-3.92593,-105.241)
(-3.91792,-105.359)
(-3.90991,-105.47)
(-3.9019,-105.574)
(-3.89389,-105.671)
(-3.88589,-105.761)
(-3.87788,-105.844)
(-3.86987,-105.921)
(-3.86186,-105.991)
(-3.85385,-106.054)
(-3.84585,-106.111)
(-3.83784,-106.161)
(-3.82983,-106.206)
(-3.82182,-106.244)
(-3.81381,-106.277)
(-3.80581,-106.303)
(-3.7978,-106.324)
(-3.78979,-106.34)
(-3.78178,-106.351)
(-3.77377,-106.356)
(-3.76577,-106.356)
(-3.75776,-106.352)
(-3.74975,-106.343)
(-3.74174,-106.33)
(-3.73373,-106.313)
(-3.72573,-106.291)
(-3.71772,-106.266)
(-3.70971,-106.238)
(-3.7017,-106.206)
(-3.69369,-106.171)
(-3.68569,-106.133)
(-3.67768,-106.093)
(-3.66967,-106.05)
(-3.66166,-106.005)
(-3.65365,-105.957)
(-3.64565,-105.908)
(-3.63764,-105.858)
(-3.62963,-105.806)
(-3.62939,-105.804)
(-3.62162,-105.753)
(-3.61361,-105.699)
(-3.60561,-105.644)
(-3.5976,-105.589)
(-3.58959,-105.533)
(-3.58158,-105.477)
(-3.57357,-105.421)
(-3.56557,-105.366)
(-3.55756,-105.311)
(-3.54955,-105.256)
(-3.54154,-105.203)
(-3.53353,-105.15)
(-3.52553,-105.098)
(-3.51752,-105.047)
(-3.50951,-104.998)
(-3.5015,-104.95)
(-3.49349,-104.904)
(-3.48549,-104.86)
(-3.47748,-104.817)
(-3.46947,-104.777)
(-3.46146,-104.738)
(-3.45345,-104.701)
(-3.44545,-104.667)
(-3.43744,-104.635)
(-3.42943,-104.605)
(-3.42142,-104.577)
(-3.41341,-104.552)
(-3.40541,-104.529)
(-3.3974,-104.508)
(-3.38939,-104.49)
(-3.38138,-104.474)
(-3.37337,-104.46)
(-3.36537,-104.449)
(-3.35736,-104.44)
(-3.34935,-104.433)
(-3.34134,-104.429)
(-3.33333,-104.426)
(-3.32533,-104.426)
(-3.31732,-104.428)
(-3.30931,-104.431)
(-3.3013,-104.437)
(-3.29329,-104.444)
(-3.28529,-104.453)
(-3.27728,-104.463)
(-3.26927,-104.475)
(-3.26126,-104.489)
(-3.25325,-104.503)
(-3.24525,-104.519)
(-3.23724,-104.536)
(-3.22923,-104.553)
(-3.22122,-104.572)
(-3.21534,-104.586)
(-3.21321,-104.591)
(-3.20521,-104.611)
(-3.1972,-104.631)
(-3.18919,-104.652)
(-3.18118,-104.672)
(-3.17317,-104.693)
(-3.16517,-104.714)
(-3.15716,-104.735)
(-3.14915,-104.756)
(-3.14114,-104.776)
(-3.13313,-104.796)
(-3.12513,-104.816)
(-3.11712,-104.835)
(-3.10911,-104.853)
(-3.1011,-104.87)
(-3.09309,-104.887)
(-3.08509,-104.903)
(-3.07708,-104.918)
(-3.06907,-104.932)
(-3.06106,-104.945)
(-3.05305,-104.957)
(-3.04505,-104.968)
(-3.03704,-104.978)
(-3.02903,-104.987)
(-3.02102,-104.994)
(-3.01301,-105.001)
(-3.00501,-105.006)
(-2.997,-105.011)
(-2.98899,-105.014)
(-2.98098,-105.016)
(-2.97297,-105.017)
(-2.96496,-105.017)
(-2.95696,-105.016)
(-2.94895,-105.014)
(-2.94094,-105.011)
(-2.93293,-105.008)
(-2.92492,-105.004)
(-2.91692,-104.999)
(-2.90891,-104.993)
(-2.9009,-104.987)
(-2.89289,-104.98)
(-2.88488,-104.973)
(-2.87688,-104.966)
(-2.87185,-104.961)
(-2.86887,-104.958)
(-2.86086,-104.95)
(-2.85285,-104.942)
(-2.84484,-104.934)
(-2.83684,-104.925)
(-2.82883,-104.917)
(-2.82082,-104.91)
(-2.81281,-104.902)
(-2.8048,-104.894)
(-2.7968,-104.887)
(-2.78879,-104.881)
(-2.78078,-104.875)
(-2.77277,-104.869)
(-2.76476,-104.864)
(-2.75676,-104.86)
(-2.74875,-104.856)
(-2.74074,-104.853)
(-2.73273,-104.85)
(-2.72472,-104.849)
(-2.71672,-104.848)
(-2.70871,-104.847)
(-2.7007,-104.848)
(-2.69269,-104.849)
(-2.68468,-104.851)
(-2.67668,-104.854)
(-2.66867,-104.858)
(-2.66066,-104.862)
(-2.65265,-104.867)
(-2.64464,-104.873)
(-2.63664,-104.879)
(-2.62863,-104.886)
(-2.62062,-104.894)
(-2.61261,-104.902)
(-2.6046,-104.91)
(-2.5966,-104.919)
(-2.58859,-104.928)
(-2.58058,-104.938)
(-2.57257,-104.947)
(-2.56456,-104.957)
(-2.55656,-104.967)
(-2.5526,-104.972)
(-2.54855,-104.977)
(-2.54054,-104.987)
(-2.53253,-104.997)
(-2.52452,-105.006)
(-2.51652,-105.016)
(-2.50851,-105.025)
(-2.5005,-105.034)
(-2.49249,-105.042)
(-2.48448,-105.05)
(-2.47648,-105.058)
(-2.46847,-105.065)
(-2.46046,-105.071)
(-2.45245,-105.077)
(-2.44444,-105.082)
(-2.43644,-105.086)
(-2.42843,-105.09)
(-2.42042,-105.093)
(-2.41241,-105.095)
(-2.4044,-105.096)
(-2.3964,-105.097)
(-2.38839,-105.097)
(-2.38038,-105.095)
(-2.37237,-105.094)
(-2.36436,-105.091)
(-2.35636,-105.088)
(-2.34835,-105.083)
(-2.34034,-105.079)
(-2.33233,-105.073)
(-2.32432,-105.067)
(-2.31632,-105.06)
(-2.30831,-105.053)
(-2.3003,-105.045)
(-2.29229,-105.037)
(-2.28428,-105.028)
(-2.27628,-105.019)
(-2.26827,-105.01)
(-2.26026,-105.001)
(-2.25225,-104.991)
(-2.24424,-104.981)
(-2.23711,-104.973)
(-2.23624,-104.972)
(-2.22823,-104.962)
(-2.22022,-104.953)
(-2.21221,-104.943)
(-2.2042,-104.934)
(-2.1962,-104.925)
(-2.18819,-104.917)
(-2.18018,-104.909)
(-2.17217,-104.901)
(-2.16416,-104.894)
(-2.15616,-104.888)
(-2.14815,-104.882)
(-2.14014,-104.877)
(-2.13213,-104.872)
(-2.12412,-104.868)
(-2.11612,-104.866)
(-2.10811,-104.863)
(-2.1001,-104.862)
(-2.09209,-104.862)
(-2.08408,-104.862)
(-2.07608,-104.863)
(-2.06807,-104.865)
(-2.06006,-104.868)
(-2.05205,-104.872)
(-2.04404,-104.877)
(-2.03604,-104.882)
(-2.02803,-104.888)
(-2.02002,-104.895)
(-2.01201,-104.903)
(-2.004,-104.911)
(-1.996,-104.92)
(-1.98799,-104.929)
(-1.97998,-104.939)
(-1.97197,-104.95)
(-1.96396,-104.96)
(-1.95596,-104.972)
(-1.94795,-104.983)
(-1.93994,-104.994)
(-1.93193,-105.006)
(-1.92392,-105.018)
(-1.91747,-105.027)
(-1.91592,-105.029)
(-1.90791,-105.041)
(-1.8999,-105.053)
(-1.89189,-105.064)
(-1.88388,-105.075)
(-1.87588,-105.085)
(-1.86787,-105.095)
(-1.85986,-105.105)
(-1.85185,-105.114)
(-1.84384,-105.122)
(-1.83584,-105.13)
(-1.82783,-105.137)
(-1.81982,-105.144)
(-1.81181,-105.149)
(-1.8038,-105.154)
(-1.7958,-105.157)
(-1.78779,-105.16)
(-1.77978,-105.162)
(-1.77177,-105.163)
(-1.76376,-105.163)
(-1.75576,-105.162)
(-1.74775,-105.16)
(-1.73974,-105.157)
(-1.73173,-105.153)
(-1.72372,-105.148)
(-1.71572,-105.143)
(-1.70771,-105.136)
(-1.6997,-105.129)
(-1.69169,-105.12)
(-1.68368,-105.111)
(-1.67568,-105.102)
(-1.66767,-105.091)
(-1.65966,-105.08)
(-1.65165,-105.069)
(-1.64364,-105.057)
(-1.63564,-105.044)
(-1.62763,-105.032)
(-1.61962,-105.019)
(-1.61161,-105.005)
(-1.6036,-104.992)
(-1.5956,-104.979)
(-1.58953,-104.968)
(-1.58759,-104.965)
(-1.57958,-104.952)
(-1.57157,-104.939)
(-1.56356,-104.926)
(-1.55556,-104.914)
(-1.54755,-104.902)
(-1.53954,-104.891)
(-1.53153,-104.88)
(-1.52352,-104.87)
(-1.51552,-104.86)
(-1.50751,-104.852)
(-1.4995,-104.844)
(-1.49149,-104.837)
(-1.48348,-104.831)
(-1.47548,-104.826)
(-1.46747,-104.822)
(-1.45946,-104.819)
(-1.45145,-104.817)
(-1.44344,-104.817)
(-1.43544,-104.817)
(-1.42743,-104.819)
(-1.41942,-104.822)
(-1.41141,-104.825)
(-1.4034,-104.83)
(-1.3954,-104.837)
(-1.38739,-104.844)
(-1.37938,-104.852)
(-1.37137,-104.862)
(-1.36336,-104.872)
(-1.35536,-104.883)
(-1.34735,-104.895)
(-1.33934,-104.909)
(-1.33133,-104.922)
(-1.32332,-104.937)
(-1.31532,-104.952)
(-1.30731,-104.968)
(-1.2993,-104.984)
(-1.29129,-105.001)
(-1.28328,-105.018)
(-1.27528,-105.036)
(-1.26727,-105.053)
(-1.25926,-105.071)
(-1.25125,-105.089)
(-1.25031,-105.091)
(-1.24324,-105.106)
(-1.23524,-105.124)
(-1.22723,-105.141)
(-1.21922,-105.158)
(-1.21121,-105.174)
(-1.2032,-105.19)
(-1.1952,-105.205)
(-1.18719,-105.22)
(-1.17918,-105.234)
(-1.17117,-105.247)
(-1.16316,-105.259)
(-1.15516,-105.27)
(-1.14715,-105.28)
(-1.13914,-105.289)
(-1.13113,-105.297)
(-1.12312,-105.304)
(-1.11512,-105.31)
(-1.10711,-105.314)
(-1.0991,-105.317)
(-1.09109,-105.319)
(-1.08308,-105.32)
(-1.07508,-105.319)
(-1.06707,-105.317)
(-1.05906,-105.314)
(-1.05105,-105.309)
(-1.04304,-105.304)
(-1.03504,-105.297)
(-1.02703,-105.288)
(-1.01902,-105.279)
(-1.01101,-105.269)
(-1.003,-105.258)
(-0.994995,-105.245)
(-0.986987,-105.232)
(-0.978979,-105.218)
(-0.970971,-105.203)
(-0.962963,-105.188)
(-0.954955,-105.172)
(-0.946947,-105.156)
(-0.938939,-105.139)
(-0.930931,-105.122)
(-0.922923,-105.104)
(-0.914915,-105.087)
(-0.906907,-105.069)
(-0.898899,-105.052)
(-0.898272,-105.051)
(-0.890891,-105.035)
(-0.882883,-105.018)
(-0.874875,-105.002)
(-0.866867,-104.986)
(-0.858859,-104.971)
(-0.850851,-104.957)
(-0.842843,-104.943)
(-0.834835,-104.93)
(-0.826827,-104.919)
(-0.818819,-104.908)
(-0.810811,-104.899)
(-0.802803,-104.89)
(-0.794795,-104.884)
(-0.786787,-104.878)
(-0.778779,-104.874)
(-0.770771,-104.872)
(-0.762763,-104.871)
(-0.754755,-104.872)
(-0.746747,-104.874)
(-0.738739,-104.879)
(-0.730731,-104.885)
(-0.722723,-104.892)
(-0.714715,-104.902)
(-0.706707,-104.913)
(-0.698699,-104.926)
(-0.690691,-104.941)
(-0.682683,-104.957)
(-0.674675,-104.975)
(-0.666667,-104.995)
(-0.658659,-105.016)
(-0.650651,-105.039)
(-0.642643,-105.064)
(-0.634635,-105.09)
(-0.626627,-105.117)
(-0.618619,-105.146)
(-0.610611,-105.176)
(-0.602603,-105.207)
(-0.594595,-105.239)
(-0.586587,-105.273)
(-0.578579,-105.307)
(-0.570571,-105.342)
(-0.562563,-105.378)
(-0.554555,-105.414)
(-0.546547,-105.451)
(-0.538539,-105.489)
(-0.530531,-105.526)
(-0.52875,-105.535)
(-0.522523,-105.564)
(-0.514515,-105.602)
(-0.506507,-105.64)
(-0.498498,-105.678)
(-0.49049,-105.716)
(-0.482482,-105.753)
(-0.474474,-105.79)
(-0.466466,-105.826)
(-0.458458,-105.862)
(-0.45045,-105.897)
(-0.442442,-105.932)
(-0.434434,-105.966)
(-0.426426,-105.998)
(-0.418418,-106.03)
(-0.41041,-106.061)
(-0.402402,-106.091)
(-0.394394,-106.12)
(-0.386386,-106.147)
(-0.378378,-106.174)
(-0.37037,-106.199)
(-0.362362,-106.223)
(-0.354354,-106.246)
(-0.346346,-106.268)
(-0.338338,-106.288)
(-0.33033,-106.308)
(-0.322322,-106.326)
(-0.314314,-106.344)
(-0.306306,-106.36)
(-0.298298,-106.375)
(-0.29029,-106.39)
(-0.282282,-106.404)
(-0.274274,-106.417)
(-0.266266,-106.429)
(-0.258258,-106.441)
(-0.25025,-106.453)
(-0.242242,-106.464)
(-0.234234,-106.475)
(-0.226226,-106.486)
(-0.218218,-106.498)
(-0.21021,-106.509)
(-0.202202,-106.521)
(-0.194194,-106.534)
(-0.186186,-106.547)
(-0.178178,-106.561)
(-0.17017,-106.577)
(-0.162162,-106.593)
(-0.154154,-106.611)
(-0.147558,-106.628)
(-0.146146,-106.631)
(-0.138138,-106.653)
(-0.13013,-106.676)
(-0.122122,-106.702)
(-0.114114,-106.73)
(-0.106106,-106.761)
(-0.0980981,-106.795)
(-0.0900901,-106.831)
(-0.0820821,-106.871)
(-0.0740741,-106.914)
(-0.0660661,-106.96)
(-0.0580581,-107.01)
(-0.0500501,-107.064)
(-0.042042,-107.122)
(-0.034034,-107.185)
(-0.026026,-107.251)
(-0.018018,-107.322)
(-0.01001,-107.398)
(-0.002002,-107.479)
(0.00600601,-107.565)
(0.014014,-107.656)
(0.022022,-107.752)
(0.03003,-107.854)
(0.038038,-107.961)
(0.046046,-108.073)
(0.0540541,-108.191)
(0.0620621,-108.316)
(0.0700701,-108.446)
(0.0780781,-108.581)
(0.0860861,-108.723)
(0.0940941,-108.871)
(0.102102,-109.025)
(0.11011,-109.186)
(0.118118,-109.352)
(0.126126,-109.525)
(0.134134,-109.703)
(0.142142,-109.888)
(0.15015,-110.08)
(0.158158,-110.277)
(0.166166,-110.48)
(0.174174,-110.69)
(0.182182,-110.905)
(0.19019,-111.127)
(0.198198,-111.355)
(0.206206,-111.588)
(0.214214,-111.827)
(0.222222,-112.072)
(0.23023,-112.322)
(0.238238,-112.578)
(0.246246,-112.839)
(0.254254,-113.106)
(0.262262,-113.377)
(0.27027,-113.654)
(0.278278,-113.935)
(0.286286,-114.221)
(0.294294,-114.512)
(0.302302,-114.807)
(0.31031,-115.106)
(0.318318,-115.409)
(0.326326,-115.716)
(0.334334,-116.027)
(0.342342,-116.341)
(0.35035,-116.659)
(0.358358,-116.979)
(0.360731,-117.075)
(0.366366,-117.303)
(0.374374,-117.629)
(0.382382,-117.958)
(0.39039,-118.29)
(0.398398,-118.623)
(0.406406,-118.959)
(0.414414,-119.296)
(0.422422,-119.635)
(0.43043,-119.975)
(0.438438,-120.317)
(0.446446,-120.659)
(0.454454,-121.003)
(0.462462,-121.347)
(0.47047,-121.691)
(0.478478,-122.036)
(0.486486,-122.381)
(0.494494,-122.726)
(0.502503,-123.07)
(0.510511,-123.415)
(0.518519,-123.758)
(0.526527,-124.101)
(0.534535,-124.443)
(0.542543,-124.784)
(0.550551,-125.124)
(0.558559,-125.463)
(0.566567,-125.8)
(0.574575,-126.136)
(0.582583,-126.47)
(0.590591,-126.802)
(0.598599,-127.132)
(0.606607,-127.461)
(0.614615,-127.787)
(0.622623,-128.11)
(0.630631,-128.432)
(0.638639,-128.751)
(0.646647,-129.068)
(0.654655,-129.381)
(0.662663,-129.693)
(0.670671,-130.001)
(0.678679,-130.307)
(0.686687,-130.61)
(0.694695,-130.91)
(0.702703,-131.207)
(0.710711,-131.501)
(0.718719,-131.792)
(0.726727,-132.079)
(0.734735,-132.364)
(0.742743,-132.645)
(0.750751,-132.924)
(0.758759,-133.199)
(0.766767,-133.47)
(0.774775,-133.739)
(0.782783,-134.004)
(0.790791,-134.266)
(0.798799,-134.524)
(0.806807,-134.78)
(0.814815,-135.032)
(0.822823,-135.28)
(0.830831,-135.525)
(0.838839,-135.767)
(0.846847,-136.006)
(0.854855,-136.241)
(0.862863,-136.473)
(0.870871,-136.702)
(0.878879,-136.928)
(0.886887,-137.15)
(0.894895,-137.369)
(0.902903,-137.585)
(0.910911,-137.798)
(0.918919,-138.007)
(0.926927,-138.213)
(0.934935,-138.417)
(0.942943,-138.617)
(0.950951,-138.814)
(0.958959,-139.008)
(0.966967,-139.199)
(0.974975,-139.387)
(0.982983,-139.572)
(0.990991,-139.754)
(0.998999,-139.933)
(1.00701,-140.11)
(1.01502,-140.283)
(1.02302,-140.454)
(1.03103,-140.622)
(1.03904,-140.787)
(1.04705,-140.95)
(1.05506,-141.11)
(1.06306,-141.267)
(1.07107,-141.422)
(1.07908,-141.574)
(1.08709,-141.723)
(1.0951,-141.87)
(1.1031,-142.015)
(1.11111,-142.157)
(1.11912,-142.297)
(1.12713,-142.434)
(1.13514,-142.569)
(1.14314,-142.702)
(1.15115,-142.832)
(1.15916,-142.96)
(1.16717,-143.086)
(1.17518,-143.21)
(1.18318,-143.332)
(1.19119,-143.452)
(1.1992,-143.569)
(1.20721,-143.685)
(1.21522,-143.798)
(1.22322,-143.91)
(1.23123,-144.019)
(1.23924,-144.127)
(1.24725,-144.233)
(1.25526,-144.337)
(1.26326,-144.439)
(1.27127,-144.539)
(1.27928,-144.638)
(1.28729,-144.735)
(1.2953,-144.83)
(1.3033,-144.923)
(1.31131,-145.015)
(1.31932,-145.105)
(1.32733,-145.194)
(1.33534,-145.281)
(1.34334,-145.366)
(1.35135,-145.45)
(1.35936,-145.533)
(1.36737,-145.614)
(1.37538,-145.693)
(1.38338,-145.771)
(1.39139,-145.848)
(1.3994,-145.923)
(1.40741,-145.997)
(1.41542,-146.07)
(1.42342,-146.141)
(1.43143,-146.211)
(1.43944,-146.28)
(1.44745,-146.348)
(1.45546,-146.414)
(1.46346,-146.479)
(1.47147,-146.543)
(1.47948,-146.606)
(1.48749,-146.668)
(1.4955,-146.728)
(1.5035,-146.788)
(1.51151,-146.846)
(1.51952,-146.904)
(1.52753,-146.96)
(1.53554,-147.015)
(1.54354,-147.07)
(1.55155,-147.123)
(1.55956,-147.175)
(1.56757,-147.227)
(1.57558,-147.277)
(1.58358,-147.327)
(1.59159,-147.376)
(1.5996,-147.424)
(1.60761,-147.47)
(1.61562,-147.517)
(1.62362,-147.562)
(1.63163,-147.606)
(1.63964,-147.65)
(1.64765,-147.693)
(1.65566,-147.735)
(1.66366,-147.776)
(1.67167,-147.817)
(1.67968,-147.856)
(1.68769,-147.896)
(1.6957,-147.934)
(1.7037,-147.972)
(1.71171,-148.009)
(1.71972,-148.045)
(1.72773,-148.081)
(1.73574,-148.116)
(1.74374,-148.15)
(1.75175,-148.184)
(1.75976,-148.217)
(1.76777,-148.249)
(1.77578,-148.281)
(1.78378,-148.313)
(1.79179,-148.344)
(1.7998,-148.374)
(1.80781,-148.403)
(1.81582,-148.433)
(1.82382,-148.461)
(1.83183,-148.489)
(1.83984,-148.517)
(1.84785,-148.544)
(1.85586,-148.571)
(1.86386,-148.597)
(1.87187,-148.622)
(1.87988,-148.647)
(1.88789,-148.672)
(1.8959,-148.696)
(1.9039,-148.72)
(1.91191,-148.743)
(1.91992,-148.766)
(1.92793,-148.789)
(1.93594,-148.811)
(1.94394,-148.833)
(1.95195,-148.854)
(1.95996,-148.875)
(1.96797,-148.896)
(1.97598,-148.916)
(1.98398,-148.936)
(1.99199,-148.955)
(2,-148.974)
};

==> walApproxImpulse-Table.tex <==
\filldraw[red] (0,0) circle(2pt);
\draw[red] [very thick] (0,0)--(0,0);
\filldraw[red] (0.13,1.99983) circle(2pt);
\draw[red] [very thick] (0.13,0)--(0.13,1.99983);
\filldraw[red] (0.26,0.830857) circle(2pt);
\draw[red] [very thick] (0.26,0)--(0.26,0.830857);
\filldraw[red] (0.39,0.626101) circle(2pt);
\draw[red] [very thick] (0.39,0)--(0.39,0.626101);
\filldraw[red] (0.52,0.538606) circle(2pt);
\draw[red] [very thick] (0.52,0)--(0.52,0.538606);
\filldraw[red] (0.65,0.477971) circle(2pt);
\draw[red] [very thick] (0.65,0)--(0.65,0.477971);
\filldraw[red] (0.78,0.431334) circle(2pt);
\draw[red] [very thick] (0.78,0)--(0.78,0.431334);
\filldraw[red] (0.91,0.394602) circle(2pt);
\draw[red] [very thick] (0.91,0)--(0.91,0.394602);
\filldraw[red] (1.04,0.365278) circle(2pt);
\draw[red] [very thick] (1.04,0)--(1.04,0.365278);
\filldraw[red] (1.17,0.341556) circle(2pt);
\draw[red] [very thick] (1.17,0)--(1.17,0.341556);
\filldraw[red] (1.3,0.322091) circle(2pt);
\draw[red] [very thick] (1.3,0)--(1.3,0.322091);
\filldraw[red] (1.43,0.305881) circle(2pt);
\draw[red] [very thick] (1.43,0)--(1.43,0.305881);
\filldraw[red] (1.56,0.292173) circle(2pt);
\draw[red] [very thick] (1.56,0)--(1.56,0.292173);
\filldraw[red] (1.69,0.280405) circle(2pt);
\draw[red] [very thick] (1.69,0)--(1.69,0.280405);
\filldraw[red] (1.82,0.270154) circle(2pt);
\draw[red] [very thick] (1.82,0)--(1.82,0.270154);
\filldraw[red] (1.95,0.261101) circle(2pt);
\draw[red] [very thick] (1.95,0)--(1.95,0.261101);
\filldraw[red] (2.08,0.253006) circle(2pt);
\draw[red] [very thick] (2.08,0)--(2.08,0.253006);
\filldraw[red] (2.21,0.245685) circle(2pt);
\draw[red] [very thick] (2.21,0)--(2.21,0.245685);
\filldraw[red] (2.34,0.239001) circle(2pt);
\draw[red] [very thick] (2.34,0)--(2.34,0.239001);
\filldraw[red] (2.47,0.232846) circle(2pt);
\draw[red] [very thick] (2.47,0)--(2.47,0.232846);
\filldraw[red] (2.6,0.227139) circle(2pt);
\draw[red] [very thick] (2.6,0)--(2.6,0.227139);
\filldraw[red] (2.73,0.221815) circle(2pt);
\draw[red] [very thick] (2.73,0)--(2.73,0.221815);
\filldraw[red] (2.86,0.216824) circle(2pt);
\draw[red] [very thick] (2.86,0)--(2.86,0.216824);
\filldraw[red] (2.99,0.212126) circle(2pt);
\draw[red] [very thick] (2.99,0)--(2.99,0.212126);
\filldraw[red] (3.12,0.20769) circle(2pt);
\draw[red] [very thick] (3.12,0)--(3.12,0.20769);
\filldraw[red] (3.25,0.203489) circle(2pt);
\draw[red] [very thick] (3.25,0)--(3.25,0.203489);
\filldraw[red] (3.38,0.199501) circle(2pt);
\draw[red] [very thick] (3.38,0)--(3.38,0.199501);
\filldraw[red] (3.51,0.195709) circle(2pt);
\draw[red] [very thick] (3.51,0)--(3.51,0.195709);
\filldraw[red] (3.64,0.192098) circle(2pt);
\draw[red] [very thick] (3.64,0)--(3.64,0.192098);
\filldraw[red] (3.77,0.188654) circle(2pt);
\draw[red] [very thick] (3.77,0)--(3.77,0.188654);
\filldraw[red] (3.9,0.185365) circle(2pt);
\draw[red] [very thick] (3.9,0)--(3.9,0.185365);
\filldraw[red] (4.03,0.182222) circle(2pt);
\draw[red] [very thick] (4.03,0)--(4.03,0.182222);
\filldraw[red] (4.16,0.179216) circle(2pt);
\draw[red] [very thick] (4.16,0)--(4.16,0.179216);
\filldraw[red] (4.29,0.176338) circle(2pt);
\draw[red] [very thick] (4.29,0)--(4.29,0.176338);
\filldraw[red] (4.42,0.17358) circle(2pt);
\draw[red] [very thick] (4.42,0)--(4.42,0.17358);
\filldraw[red] (4.55,0.170937) circle(2pt);
\draw[red] [very thick] (4.55,0)--(4.55,0.170937);
\filldraw[red] (4.68,0.168401) circle(2pt);
\draw[red] [very thick] (4.68,0)--(4.68,0.168401);
\filldraw[red] (4.81,0.165968) circle(2pt);
\draw[red] [very thick] (4.81,0)--(4.81,0.165968);
\filldraw[red] (4.94,0.163631) circle(2pt);
\draw[red] [very thick] (4.94,0)--(4.94,0.163631);
\filldraw[red] (5.07,0.161385) circle(2pt);
\draw[red] [very thick] (5.07,0)--(5.07,0.161385);
\filldraw[red] (5.2,0.159225) circle(2pt);
\draw[red] [very thick] (5.2,0)--(5.2,0.159225);
\filldraw[red] (5.33,0.157148) circle(2pt);
\draw[red] [very thick] (5.33,0)--(5.33,0.157148);
\filldraw[red] (5.46,0.155149) circle(2pt);
\draw[red] [very thick] (5.46,0)--(5.46,0.155149);
\filldraw[red] (5.59,0.153224) circle(2pt);
\draw[red] [very thick] (5.59,0)--(5.59,0.153224);
\filldraw[red] (5.72,0.151369) circle(2pt);
\draw[red] [very thick] (5.72,0)--(5.72,0.151369);
\filldraw[red] (5.85,0.149581) circle(2pt);
\draw[red] [very thick] (5.85,0)--(5.85,0.149581);
\filldraw[red] (5.98,0.147856) circle(2pt);
\draw[red] [very thick] (5.98,0)--(5.98,0.147856);
\filldraw[red] (6.11,0.146192) circle(2pt);
\draw[red] [very thick] (6.11,0)--(6.11,0.146192);
\filldraw[red] (6.24,0.144584) circle(2pt);
\draw[red] [very thick] (6.24,0)--(6.24,0.144584);
\filldraw[red] (6.37,0.143032) circle(2pt);
\draw[red] [very thick] (6.37,0)--(6.37,0.143032);
\filldraw[red] (6.5,0.141531) circle(2pt);
\draw[red] [very thick] (6.5,0)--(6.5,0.141531);
\filldraw[red] (6.63,0.14008) circle(2pt);
\draw[red] [very thick] (6.63,0)--(6.63,0.14008);
\filldraw[red] (6.76,0.138676) circle(2pt);
\draw[red] [very thick] (6.76,0)--(6.76,0.138676);
\filldraw[red] (6.89,0.137317) circle(2pt);
\draw[red] [very thick] (6.89,0)--(6.89,0.137317);
\filldraw[red] (7.02,0.136) circle(2pt);
\draw[red] [very thick] (7.02,0)--(7.02,0.136);
\filldraw[red] (7.15,0.134724) circle(2pt);
\draw[red] [very thick] (7.15,0)--(7.15,0.134724);
\filldraw[red] (7.28,0.133486) circle(2pt);
\draw[red] [very thick] (7.28,0)--(7.28,0.133486);
\filldraw[red] (7.41,0.132286) circle(2pt);
\draw[red] [very thick] (7.41,0)--(7.41,0.132286);
\filldraw[red] (7.54,0.131121) circle(2pt);
\draw[red] [very thick] (7.54,0)--(7.54,0.131121);
\filldraw[red] (7.67,0.129989) circle(2pt);
\draw[red] [very thick] (7.67,0)--(7.67,0.129989);
\filldraw[red] (7.8,0.12889) circle(2pt);
\draw[red] [very thick] (7.8,0)--(7.8,0.12889);
\filldraw[red] (7.93,0.127821) circle(2pt);
\draw[red] [very thick] (7.93,0)--(7.93,0.127821);
\filldraw[red] (8.06,0.126781) circle(2pt);
\draw[red] [very thick] (8.06,0)--(8.06,0.126781);
\filldraw[red] (8.19,0.125769) circle(2pt);
\draw[red] [very thick] (8.19,0)--(8.19,0.125769);
\filldraw[red] (8.32,0.124784) circle(2pt);
\draw[red] [very thick] (8.32,0)--(8.32,0.124784);
\filldraw[red] (8.45,0.123825) circle(2pt);
\draw[red] [very thick] (8.45,0)--(8.45,0.123825);
\filldraw[red] (8.58,0.12289) circle(2pt);
\draw[red] [very thick] (8.58,0)--(8.58,0.12289);
\filldraw[red] (8.71,0.121978) circle(2pt);
\draw[red] [very thick] (8.71,0)--(8.71,0.121978);
\filldraw[red] (8.84,0.121089) circle(2pt);
\draw[red] [very thick] (8.84,0)--(8.84,0.121089);
\filldraw[red] (8.97,0.120221) circle(2pt);
\draw[red] [very thick] (8.97,0)--(8.97,0.120221);
\filldraw[red] (9.1,0.119373) circle(2pt);
\draw[red] [very thick] (9.1,0)--(9.1,0.119373);
\filldraw[red] (9.23,0.118545) circle(2pt);
\draw[red] [very thick] (9.23,0)--(9.23,0.118545);
\filldraw[red] (9.36,0.117737) circle(2pt);
\draw[red] [very thick] (9.36,0)--(9.36,0.117737);
\filldraw[red] (9.49,0.116946) circle(2pt);
\draw[red] [very thick] (9.49,0)--(9.49,0.116946);
\filldraw[red] (9.62,0.116172) circle(2pt);
\draw[red] [very thick] (9.62,0)--(9.62,0.116172);
\filldraw[red] (9.75,0.115415) circle(2pt);
\draw[red] [very thick] (9.75,0)--(9.75,0.115415);
\filldraw[red] (9.88,0.114674) circle(2pt);
\draw[red] [very thick] (9.88,0)--(9.88,0.114674);
\filldraw[red] (10.01,0.113949) circle(2pt);
\draw[red] [very thick] (10.01,0)--(10.01,0.113949);
\filldraw[red] (10.14,0.113238) circle(2pt);
\draw[red] [very thick] (10.14,0)--(10.14,0.113238);
\filldraw[red] (10.27,0.112541) circle(2pt);
\draw[red] [very thick] (10.27,0)--(10.27,0.112541);
\filldraw[red] (10.4,0.111859) circle(2pt);
\draw[red] [very thick] (10.4,0)--(10.4,0.111859);
\filldraw[red] (10.53,0.111189) circle(2pt);
\draw[red] [very thick] (10.53,0)--(10.53,0.111189);
\filldraw[red] (10.66,0.110532) circle(2pt);
\draw[red] [very thick] (10.66,0)--(10.66,0.110532);
\filldraw[red] (10.79,0.109887) circle(2pt);
\draw[red] [very thick] (10.79,0)--(10.79,0.109887);
\filldraw[red] (10.92,0.109254) circle(2pt);
\draw[red] [very thick] (10.92,0)--(10.92,0.109254);
\filldraw[red] (11.05,0.108632) circle(2pt);
\draw[red] [very thick] (11.05,0)--(11.05,0.108632);
\filldraw[red] (11.18,0.108022) circle(2pt);
\draw[red] [very thick] (11.18,0)--(11.18,0.108022);
\filldraw[red] (11.31,0.107421) circle(2pt);
\draw[red] [very thick] (11.31,0)--(11.31,0.107421);
\filldraw[red] (11.44,0.106832) circle(2pt);
\draw[red] [very thick] (11.44,0)--(11.44,0.106832);
\filldraw[red] (11.57,0.106252) circle(2pt);
\draw[red] [very thick] (11.57,0)--(11.57,0.106252);
\filldraw[red] (11.7,0.105681) circle(2pt);
\draw[red] [very thick] (11.7,0)--(11.7,0.105681);
\filldraw[red] (11.83,0.10512) circle(2pt);
\draw[red] [very thick] (11.83,0)--(11.83,0.10512);
\filldraw[red] (11.96,0.104568) circle(2pt);
\draw[red] [very thick] (11.96,0)--(11.96,0.104568);
\filldraw[red] (12.09,0.104024) circle(2pt);
\draw[red] [very thick] (12.09,0)--(12.09,0.104024);
\filldraw[red] (12.22,0.103489) circle(2pt);
\draw[red] [very thick] (12.22,0)--(12.22,0.103489);
\filldraw[red] (12.35,0.102962) circle(2pt);
\draw[red] [very thick] (12.35,0)--(12.35,0.102962);
\filldraw[red] (12.48,0.102443) circle(2pt);
\draw[red] [very thick] (12.48,0)--(12.48,0.102443);
\filldraw[red] (12.61,0.101931) circle(2pt);
\draw[red] [very thick] (12.61,0)--(12.61,0.101931);
\filldraw[red] (12.74,0.101427) circle(2pt);
\draw[red] [very thick] (12.74,0)--(12.74,0.101427);
\filldraw[red] (12.87,0.10093) circle(2pt);
\draw[red] [very thick] (12.87,0)--(12.87,0.10093);
\filldraw[red] (13,0.100441) circle(2pt);
\draw[red] [very thick] (13,0)--(13,0.100441);

==> walburgImpulse-Table.tex <==
\filldraw [blue] (0,0) circle(2pt);
\draw [blue] [very thick] (0,0)--(0,0);
\filldraw (0.13,2) circle(2pt);
\draw [blue] [very thick] (0.13,0)--(0.13,2);
\filldraw [blue] (0.26,0.828427) circle(2pt);
\draw [blue] [very thick] (0.26,0)--(0.26,0.828427);
\filldraw [blue] (0.39,0.635674) circle(2pt);
\draw [blue] [very thick] (0.39,0)--(0.39,0.635674);
\filldraw [blue] (0.52,0.535898) circle(2pt);
\draw [blue] [very thick] (0.52,0)--(0.52,0.535898);
\filldraw [blue] (0.65,0.472136) circle(2pt);
\draw [blue] [very thick] (0.65,0)--(0.65,0.472136);
\filldraw [blue] (0.78,0.426844) circle(2pt);
\draw [blue] [very thick] (0.78,0)--(0.78,0.426844);
\filldraw [blue] (0.91,0.392523) circle(2pt);
\draw [blue] [very thick] (0.91,0)--(0.91,0.392523);
\filldraw [blue] (1.04,0.365352) circle(2pt);
\draw [blue] [very thick] (1.04,0)--(1.04,0.365352);
\filldraw [blue] (1.17,0.343146) circle(2pt);
\draw [blue] [very thick] (1.17,0)--(1.17,0.343146);
\filldraw [blue] (1.3,0.324555) circle(2pt);
\draw [blue] [very thick] (1.3,0)--(1.3,0.324555);
\filldraw [blue] (1.43,0.308694) circle(2pt);
\draw [blue] [very thick] (1.43,0)--(1.43,0.308694);
\filldraw [blue] (1.56,0.294954) circle(2pt);
\draw [blue] [very thick] (1.56,0)--(1.56,0.294954);
\filldraw [blue] (1.69,0.282899) circle(2pt);
\draw [blue] [very thick] (1.69,0)--(1.69,0.282899);
\filldraw [blue] (1.82,0.272212) circle(2pt);
\draw [blue] [very thick] (1.82,0)--(1.82,0.272212);
\filldraw [blue] (1.95,0.262652) circle(2pt);
\draw [blue] [very thick] (1.95,0)--(1.95,0.262652);
\filldraw [blue] (2.08,0.254033) circle(2pt);
\draw [blue] [very thick] (2.08,0)--(2.08,0.254033);
\filldraw [blue] (2.21,0.246211) circle(2pt);
\draw [blue] [very thick] (2.21,0)--(2.21,0.246211);
\filldraw [blue] (2.34,0.23907) circle(2pt);
\draw [blue] [very thick] (2.34,0)--(2.34,0.23907);
\filldraw [blue] (2.47,0.232517) circle(2pt);
\draw [blue] [very thick] (2.47,0)--(2.47,0.232517);
\filldraw [blue] (2.6,0.226474) circle(2pt);
\draw [blue] [very thick] (2.6,0)--(2.6,0.226474);
\filldraw [blue] (2.73,0.220879) circle(2pt);
\draw [blue] [very thick] (2.73,0)--(2.73,0.220879);
\filldraw [blue] (2.86,0.21568) circle(2pt);
\draw [blue] [very thick] (2.86,0)--(2.86,0.21568);
\filldraw [blue] (2.99,0.210832) circle(2pt);
\draw [blue] [very thick] (2.99,0)--(2.99,0.210832);
\filldraw [blue] (3.12,0.206296) circle(2pt);
\draw [blue] [very thick] (3.12,0)--(3.12,0.206296);
\filldraw [blue] (3.25,0.202041) circle(2pt);
\draw [blue] [very thick] (3.25,0)--(3.25,0.202041);
\filldraw [blue] (3.38,0.198039) circle(2pt);
\draw [blue] [very thick] (3.38,0)--(3.38,0.198039);
\filldraw [blue] (3.51,0.194266) circle(2pt);
\draw [blue] [very thick] (3.51,0)--(3.51,0.194266);
\filldraw [blue] (3.64,0.1907) circle(2pt);
\draw [blue] [very thick] (3.64,0)--(3.64,0.1907);
\filldraw [blue] (3.77,0.187324) circle(2pt);
\draw [blue] [very thick] (3.77,0)--(3.77,0.187324);
\filldraw [blue] (3.9,0.184122) circle(2pt);
\draw [blue] [very thick] (3.9,0)--(3.9,0.184122);
\filldraw [blue] (4.03,0.181078) circle(2pt);
\draw [blue] [very thick] (4.03,0)--(4.03,0.181078);
\filldraw [blue] (4.16,0.17818) circle(2pt);
\draw [blue] [very thick] (4.16,0)--(4.16,0.17818);
\filldraw [blue] (4.29,0.175417) circle(2pt);
\draw [blue] [very thick] (4.29,0)--(4.29,0.175417);
\filldraw [blue] (4.42,0.172778) circle(2pt);
\draw [blue] [very thick] (4.42,0)--(4.42,0.172778);
\filldraw [blue] (4.55,0.170256) circle(2pt);
\draw [blue] [very thick] (4.55,0)--(4.55,0.170256);
\filldraw [blue] (4.68,0.16784) circle(2pt);
\draw [blue] [very thick] (4.68,0)--(4.68,0.16784);
\filldraw [blue] (4.81,0.165525) circle(2pt);
\draw [blue] [very thick] (4.81,0)--(4.81,0.165525);
\filldraw [blue] (4.94,0.163303) circle(2pt);
\draw [blue] [very thick] (4.94,0)--(4.94,0.163303);
\filldraw [blue] (5.07,0.161168) circle(2pt);
\draw [blue] [very thick] (5.07,0)--(5.07,0.161168);
\filldraw [blue] (5.2,0.159115) circle(2pt);
\draw [blue] [very thick] (5.2,0)--(5.2,0.159115);
\filldraw [blue] (5.33,0.157138) circle(2pt);
\draw [blue] [very thick] (5.33,0)--(5.33,0.157138);
\filldraw [blue] (5.46,0.155233) circle(2pt);
\draw [blue] [very thick] (5.46,0)--(5.46,0.155233);
\filldraw [blue] (5.59,0.153396) circle(2pt);
\draw [blue] [very thick] (5.59,0)--(5.59,0.153396);
\filldraw [blue] (5.72,0.151622) circle(2pt);
\draw [blue] [very thick] (5.72,0)--(5.72,0.151622);
\filldraw [blue] (5.85,0.149909) circle(2pt);
\draw [blue] [very thick] (5.85,0)--(5.85,0.149909);
\filldraw [blue] (5.98,0.148252) circle(2pt);
\draw [blue] [very thick] (5.98,0)--(5.98,0.148252);
\filldraw [blue] (6.11,0.146649) circle(2pt);
\draw [blue] [very thick] (6.11,0)--(6.11,0.146649);
\filldraw [blue] (6.24,0.145097) circle(2pt);
\draw [blue] [very thick] (6.24,0)--(6.24,0.145097);
\filldraw [blue] (6.37,0.143594) circle(2pt);
\draw [blue] [very thick] (6.37,0)--(6.37,0.143594);
\filldraw [blue] (6.5,0.142136) circle(2pt);
\draw [blue] [very thick] (6.5,0)--(6.5,0.142136);
\filldraw [blue] (6.63,0.140721) circle(2pt);
\draw [blue] [very thick] (6.63,0)--(6.63,0.140721);
\filldraw [blue] (6.76,0.139348) circle(2pt);
\draw [blue] [very thick] (6.76,0)--(6.76,0.139348);
\filldraw [blue] (6.89,0.138015) circle(2pt);
\draw [blue] [very thick] (6.89,0)--(6.89,0.138015);
\filldraw [blue] (7.02,0.136719) circle(2pt);
\draw [blue] [very thick] (7.02,0)--(7.02,0.136719);
\filldraw [blue] (7.15,0.135459) circle(2pt);
\draw [blue] [very thick] (7.15,0)--(7.15,0.135459);
\filldraw [blue] (7.28,0.134233) circle(2pt);
\draw [blue] [very thick] (7.28,0)--(7.28,0.134233);
\filldraw [blue] (7.41,0.133039) circle(2pt);
\draw [blue] [very thick] (7.41,0)--(7.41,0.133039);
\filldraw [blue] (7.54,0.131877) circle(2pt);
\draw [blue] [very thick] (7.54,0)--(7.54,0.131877);
\filldraw [blue] (7.67,0.130745) circle(2pt);
\draw [blue] [very thick] (7.67,0)--(7.67,0.130745);
\filldraw [blue] (7.8,0.129642) circle(2pt);
\draw [blue] [very thick] (7.8,0)--(7.8,0.129642);
\filldraw [blue] (7.93,0.128566) circle(2pt);
\draw [blue] [very thick] (7.93,0)--(7.93,0.128566);
\filldraw [blue] (8.06,0.127516) circle(2pt);
\draw [blue] [very thick] (8.06,0)--(8.06,0.127516);
\filldraw [blue] (8.19,0.126492) circle(2pt);
\draw [blue] [very thick] (8.19,0)--(8.19,0.126492);
\filldraw [blue] (8.32,0.125492) circle(2pt);
\draw [blue] [very thick] (8.32,0)--(8.32,0.125492);
\filldraw [blue] (8.45,0.124515) circle(2pt);
\draw [blue] [very thick] (8.45,0)--(8.45,0.124515);
\filldraw [blue] (8.58,0.123561) circle(2pt);
\draw [blue] [very thick] (8.58,0)--(8.58,0.123561);
\filldraw [blue] (8.71,0.122629) circle(2pt);
\draw [blue] [very thick] (8.71,0)--(8.71,0.122629);
\filldraw [blue] (8.84,0.121717) circle(2pt);
\draw [blue] [very thick] (8.84,0)--(8.84,0.121717);
\filldraw [blue] (8.97,0.120825) circle(2pt);
\draw [blue] [very thick] (8.97,0)--(8.97,0.120825);
\filldraw [blue] (9.1,0.119953) circle(2pt);
\draw [blue] [very thick] (9.1,0)--(9.1,0.119953);
\filldraw [blue] (9.23,0.119099) circle(2pt);
\draw [blue] [very thick] (9.23,0)--(9.23,0.119099);
\filldraw [blue] (9.36,0.118263) circle(2pt);
\draw [blue] [very thick] (9.36,0)--(9.36,0.118263);
\filldraw [blue] (9.49,0.117445) circle(2pt);
\draw [blue] [very thick] (9.49,0)--(9.49,0.117445);
\filldraw [blue] (9.62,0.116643) circle(2pt);
\draw [blue] [very thick] (9.62,0)--(9.62,0.116643);
\filldraw [blue] (9.75,0.115858) circle(2pt);
\draw [blue] [very thick] (9.75,0)--(9.75,0.115858);
\filldraw [blue] (9.88,0.115088) circle(2pt);
\draw [blue] [very thick] (9.88,0)--(9.88,0.115088);
\filldraw [blue] (10.01,0.114333) circle(2pt);
\draw [blue] [very thick] (10.01,0)--(10.01,0.114333);
\filldraw [blue] (10.14,0.113593) circle(2pt);
\draw [blue] [very thick] (10.14,0)--(10.14,0.113593);
\filldraw [blue] (10.27,0.112867) circle(2pt);
\draw [blue] [very thick] (10.27,0)--(10.27,0.112867);
\filldraw [blue] (10.4,0.112155) circle(2pt);
\draw [blue] [very thick] (10.4,0)--(10.4,0.112155);
\filldraw [blue] (10.53,0.111456) circle(2pt);
\draw [blue] [very thick] (10.53,0)--(10.53,0.111456);
\filldraw [blue] (10.66,0.11077) circle(2pt);
\draw [blue] [very thick] (10.66,0)--(10.66,0.11077);
\filldraw [blue] (10.79,0.110097) circle(2pt);
\draw [blue] [very thick] (10.79,0)--(10.79,0.110097);
\filldraw [blue] (10.92,0.109436) circle(2pt);
\draw [blue] [very thick] (10.92,0)--(10.92,0.109436);
\filldraw [blue] (11.05,0.108786) circle(2pt);
\draw [blue] [very thick] (11.05,0)--(11.05,0.108786);
\filldraw [blue] (11.18,0.108148) circle(2pt);
\draw [blue] [very thick] (11.18,0)--(11.18,0.108148);
\filldraw [blue] (11.31,0.107521) circle(2pt);
\draw [blue] [very thick] (11.31,0)--(11.31,0.107521);
\filldraw [blue] (11.44,0.106905) circle(2pt);
\draw [blue] [very thick] (11.44,0)--(11.44,0.106905);
\filldraw [blue] (11.57,0.106299) circle(2pt);
\draw [blue] [very thick] (11.57,0)--(11.57,0.106299);
\filldraw [blue] (11.7,0.105704) circle(2pt);
\draw [blue] [very thick] (11.7,0)--(11.7,0.105704);
\filldraw [blue] (11.83,0.105118) circle(2pt);
\draw [blue] [very thick] (11.83,0)--(11.83,0.105118);
\filldraw [blue] (11.96,0.104542) circle(2pt);
\draw [blue] [very thick] (11.96,0)--(11.96,0.104542);
\filldraw [blue] (12.09,0.103975) circle(2pt);
\draw [blue] [very thick] (12.09,0)--(12.09,0.103975);
\filldraw [blue] (12.22,0.103418) circle(2pt);
\draw [blue] [very thick] (12.22,0)--(12.22,0.103418);
\filldraw [blue] (12.35,0.102869) circle(2pt);
\draw [blue] [very thick] (12.35,0)--(12.35,0.102869);
\filldraw [blue] (12.48,0.102329) circle(2pt);
\draw [blue] [very thick] (12.48,0)--(12.48,0.102329);
\filldraw [blue] (12.61,0.101798) circle(2pt);
\draw [blue] [very thick] (12.61,0)--(12.61,0.101798);
\filldraw [blue] (12.74,0.101274) circle(2pt);
\draw [blue] [very thick] (12.74,0)--(12.74,0.101274);
\filldraw [blue] (12.87,0.100759) circle(2pt);
\draw [blue] [very thick] (12.87,0)--(12.87,0.100759);
\filldraw [blue] (13,0.100251) circle(2pt);
\draw [blue] [very thick] (13,0)--(13,0.100251);
